Improving Object Detection with Selective Self-supervised Self-training

We study how to leverage Web images to augment human-curated object detection datasets. Our approach is two-pronged. On the one hand, we retrieve Web images by image-to-image search, which incurs less domain shift from the curated data than other search methods. The Web images are diverse, supplying a wide variety of object poses, appearances, their interactions with the context, etc. On the other hand, we propose a novel learning method motivated by two parallel lines of work that explore unlabeled data for image classification: self-training and self-supervised learning. They fail to improve object detectors in their vanilla forms due to the domain gap between the Web images and curated datasets. To tackle this challenge, we propose a selective net to rectify the supervision signals in Web images. It not only identifies positive bounding boxes but also creates a safe zone for mining hard negative boxes. We report state-of-the-art results on detecting backpacks and chairs from everyday scenes, along with other challenging object classes.

==> bibitems.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{arazo2019pseudo}
Arazo, E., Ortego, D., Albert, P., O'Connor, N.E., McGuinness, K.:
  Pseudo-labeling and confirmation bias in deep semi-supervised learning. arXiv
  preprint arXiv:1908.02983  (2019)

\bibitem{arun2019dissimilarity}
Arun, A., Jawahar, C., Kumar, M.P.: Dissimilarity coefficient based weakly
  supervised object detection. In: Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition. pp. 9432--9441 (2019)

\bibitem{bachman2014learning}
Bachman, P., Alsharif, O., Precup, D.: Learning with pseudo-ensembles. In:
  Advances in neural information processing systems. pp. 3365--3373 (2014)

\bibitem{berthelot2019mixmatch}
Berthelot, D., Carlini, N., Goodfellow, I., Papernot, N., Oliver, A., Raffel,
  C.A.: Mixmatch: A holistic approach to semi-supervised learning. In: Advances
  in Neural Information Processing Systems. pp. 5050--5060 (2019)

\bibitem{bilen2016weakly}
Bilen, H., Vedaldi, A.: Weakly supervised deep detection networks. In:
  Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition. pp. 2846--2854 (2016)

\bibitem{chen2020simple}
Chen, T., Kornblith, S., Norouzi, M., Hinton, G.: A simple framework for
  contrastive learning of visual representations. arXiv preprint
  arXiv:2002.05709  (2020)

\bibitem{dai2016r}
Dai, J., Li, Y., He, K., Sun, J.: R-fcn: Object detection via region-based
  fully convolutional networks. In: Advances in neural information processing
  systems. pp. 379--387 (2016)

\bibitem{deng2009imagenet}
Deng, J., Dong, W., Socher, R., Li, L.J., Li, K., Fei-Fei, L.: Imagenet: A
  large-scale hierarchical image database. In: 2009 IEEE conference on computer
  vision and pattern recognition. pp. 248--255. Ieee (2009)

\bibitem{doersch2015unsupervised}
Doersch, C., Gupta, A., Efros, A.A.: Unsupervised visual representation
  learning by context prediction. In: Proceedings of the IEEE International
  Conference on Computer Vision. pp. 1422--1430 (2015)

\bibitem{donahue2019large}
Donahue, J., Simonyan, K.: Large scale adversarial representation learning. In:
  Advances in Neural Information Processing Systems. pp. 10541--10551 (2019)

\bibitem{everingham2010pascal}
Everingham, M., Van~Gool, L., Williams, C.K., Winn, J., Zisserman, A.: The
  pascal visual object classes (voc) challenge. International journal of
  computer vision  \textbf{88}(2),  303--338 (2010)

\bibitem{gao2019note}
Gao, J., Wang, J., Dai, S., Li, L.J., Nevatia, R.: Note-rcnn: Noise tolerant
  ensemble rcnn for semi-supervised object detection. In: Proceedings of the
  IEEE International Conference on Computer Vision. pp. 9508--9517 (2019)

\bibitem{gao2019c}
Gao, Y., Liu, B., Guo, N., Ye, X., Wan, F., You, H., Fan, D.: C-midn: Coupled
  multiple instance detection network with segmentation guidance for weakly
  supervised object detection. In: Proceedings of the IEEE International
  Conference on Computer Vision. pp. 9834--9843 (2019)

\bibitem{gidaris2018unsupervised}
Gidaris, S., Singh, P., Komodakis, N.: Unsupervised representation learning by
  predicting image rotations. arXiv preprint arXiv:1803.07728  (2018)

\bibitem{girshick2015fast}
Girshick, R.: Fast r-cnn. In: Proceedings of the IEEE international conference
  on computer vision. pp. 1440--1448 (2015)

\bibitem{grabner2011makes}
Grabner, H., Gall, J., Van~Gool, L.: What makes a chair a chair? In: CVPR 2011.
  pp. 1529--1536. IEEE (2011)

\bibitem{he2019momentum}
He, K., Fan, H., Wu, Y., Xie, S., Girshick, R.: Momentum contrast for
  unsupervised visual representation learning. arXiv preprint arXiv:1911.05722
  (2019)

\bibitem{he2017mask}
He, K., Gkioxari, G., Doll{\'a}r, P., Girshick, R.: Mask r-cnn. In: Proceedings
  of the IEEE international conference on computer vision. pp. 2961--2969
  (2017)

\bibitem{he2016deep}
He, K., Zhang, X., Ren, S., Sun, J.: Deep residual learning for image
  recognition. In: Proceedings of the IEEE conference on computer vision and
  pattern recognition. pp. 770--778 (2016)

\bibitem{iscen2019label}
Iscen, A., Tolias, G., Avrithis, Y., Chum, O.: Label propagation for deep
  semi-supervised learning. In: Proceedings of the IEEE Conference on Computer
  Vision and Pattern Recognition. pp. 5070--5079 (2019)

\bibitem{jenni2018self}
Jenni, S., Favaro, P.: Self-supervised feature learning by learning to spot
  artifacts. In: Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition. pp. 2733--2742 (2018)

\bibitem{jeong2019consistency}
Jeong, J., Lee, S., Kim, J., Kwak, N.: Consistency-based semi-supervised
  learning for object detection. In: Advances in Neural Information Processing
  Systems. pp. 10758--10767 (2019)

\bibitem{jiang2019synthetic}
Jiang, L., Huang, D., Yang, W.: Synthetic vs real: Deep learning on controlled
  noise. arXiv preprint arXiv:1911.09781  (2019)

\bibitem{kolesnikov2019large}
Kolesnikov, A., Beyer, L., Zhai, X., Puigcerver, J., Yung, J., Gelly, S.,
  Houlsby, N.: Large scale learning of general visual representations for
  transfer. arXiv preprint arXiv:1912.11370  (2019)

\bibitem{kumar2016track}
Kumar~Singh, K., Xiao, F., Jae~Lee, Y.: Track and transfer: Watching videos to
  simulate strong human supervision for weakly-supervised object detection. In:
  Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition. pp. 3548--3556 (2016)

\bibitem{laine2016temporal}
Laine, S., Aila, T.: Temporal ensembling for semi-supervised learning. arXiv
  preprint arXiv:1610.02242  (2016)

\bibitem{lee2013pseudo}
Lee, D.H.: Pseudo-label: The simple and efficient semi-supervised learning
  method for deep neural networks. In: Workshop on challenges in representation
  learning, ICML. vol.~3, p.~2 (2013)

\bibitem{lee2019multi}
Lee, W., Na, J., Kim, G.: Multi-task self-supervised object detection via
  recycling of bounding box annotations. In: Proceedings of the IEEE Conference
  on Computer Vision and Pattern Recognition. pp. 4984--4993 (2019)

\bibitem{li2019weakly}
Li, X., Kan, M., Shan, S., Chen, X.: Weakly supervised object detection with
  segmentation collaboration. In: Proceedings of the IEEE International
  Conference on Computer Vision. pp. 9735--9744 (2019)

\bibitem{lin2017feature}
Lin, T.Y., Doll{\'a}r, P., Girshick, R., He, K., Hariharan, B., Belongie, S.:
  Feature pyramid networks for object detection. In: Proceedings of the IEEE
  conference on computer vision and pattern recognition. pp. 2117--2125 (2017)

\bibitem{lin2017focal}
Lin, T.Y., Goyal, P., Girshick, R., He, K., Doll{\'a}r, P.: Focal loss for
  dense object detection. In: Proceedings of the IEEE international conference
  on computer vision. pp. 2980--2988 (2017)

\bibitem{lin2014microsoft}
Lin, T.Y., Maire, M., Belongie, S., Hays, J., Perona, P., Ramanan, D.,
  Doll{\'a}r, P., Zitnick, C.L.: Microsoft coco: Common objects in context. In:
  European conference on computer vision. pp. 740--755. Springer (2014)

\bibitem{liu2016ssd}
Liu, W., Anguelov, D., Erhan, D., Szegedy, C., Reed, S., Fu, C.Y., Berg, A.C.:
  Ssd: Single shot multibox detector. In: European conference on computer
  vision. pp. 21--37. Springer (2016)

\bibitem{luo2018smooth}
Luo, Y., Zhu, J., Li, M., Ren, Y., Zhang, B.: Smooth neighbors on teacher
  graphs for semi-supervised learning. In: Proceedings of the IEEE conference
  on computer vision and pattern recognition. pp. 8896--8905 (2018)

\bibitem{mahajan2018exploring}
Mahajan, D., Girshick, R., Ramanathan, V., He, K., Paluri, M., Li, Y.,
  Bharambe, A., van~der Maaten, L.: Exploring the limits of weakly supervised
  pretraining. In: Proceedings of the European Conference on Computer Vision
  (ECCV). pp. 181--196 (2018)

\bibitem{minsky1988society}
Minsky, M.: Society of mind. Simon and Schuster (1988)

\bibitem{miyato2018virtual}
Miyato, T., Maeda, S.i., Koyama, M., Ishii, S.: Virtual adversarial training: a
  regularization method for supervised and semi-supervised learning. IEEE
  transactions on pattern analysis and machine intelligence  \textbf{41}(8),
  1979--1993 (2018)

\bibitem{noroozi2016unsupervised}
Noroozi, M., Favaro, P.: Unsupervised learning of visual representations by
  solving jigsaw puzzles. In: European Conference on Computer Vision. pp.
  69--84. Springer (2016)

\bibitem{oliver2018realistic}
Oliver, A., Odena, A., Raffel, C.A., Cubuk, E.D., Goodfellow, I.: Realistic
  evaluation of deep semi-supervised learning algorithms. In: Advances in
  Neural Information Processing Systems. pp. 3235--3246 (2018)

\bibitem{oord2018representation}
Oord, A.v.d., Li, Y., Vinyals, O.: Representation learning with contrastive
  predictive coding. arXiv preprint arXiv:1807.03748  (2018)

\bibitem{pathak2017learning}
Pathak, D., Girshick, R., Doll{\'a}r, P., Darrell, T., Hariharan, B.: Learning
  features by watching objects move. In: Proceedings of the IEEE Conference on
  Computer Vision and Pattern Recognition. pp. 2701--2710 (2017)

\bibitem{pathak2016context}
Pathak, D., Krahenbuhl, P., Donahue, J., Darrell, T., Efros, A.A.: Context
  encoders: Feature learning by inpainting. In: Proceedings of the IEEE
  conference on computer vision and pattern recognition. pp. 2536--2544 (2016)

\bibitem{prest2012learning}
Prest, A., Leistner, C., Civera, J., Schmid, C., Ferrari, V.: Learning object
  class detectors from weakly annotated video. In: 2012 IEEE Conference on
  Computer Vision and Pattern Recognition. pp. 3282--3289. IEEE (2012)

\bibitem{rasmus2015semi}
Rasmus, A., Berglund, M., Honkala, M., Valpola, H., Raiko, T.: Semi-supervised
  learning with ladder networks. In: Advances in neural information processing
  systems. pp. 3546--3554 (2015)

\bibitem{redmon2017yolo9000}
Redmon, J., Farhadi, A.: Yolo9000: better, faster, stronger. In: Proceedings of
  the IEEE conference on computer vision and pattern recognition. pp.
  7263--7271 (2017)

\bibitem{ren2015faster}
Ren, S., He, K., Girshick, R., Sun, J.: Faster r-cnn: Towards real-time object
  detection with region proposal networks. In: Advances in neural information
  processing systems. pp. 91--99 (2015)

\bibitem{riloff2003learning}
Riloff, E., Wiebe, J.: Learning extraction patterns for subjective expressions.
  In: Proceedings of the 2003 conference on Empirical methods in natural
  language processing. pp. 105--112 (2003)

\bibitem{scudder1965probability}
Scudder, H.: Probability of error of some adaptive pattern-recognition
  machines. IEEE Transactions on Information Theory  \textbf{11}(3),  363--371
  (1965)

\bibitem{shi2018transductive}
Shi, W., Gong, Y., Ding, C., MaXiaoyu~Tao, Z., Zheng, N.: Transductive
  semi-supervised deep learning using min-max features. In: Proceedings of the
  European Conference on Computer Vision (ECCV). pp. 299--315 (2018)

\bibitem{singh2019you}
Singh, K.K., Lee, Y.J.: You reap what you sow: Using videos to generate high
  precision object proposals for weakly-supervised object detection. In:
  Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition. pp. 9414--9422 (2019)

\bibitem{tang2017multiple}
Tang, P., Wang, X., Bai, X., Liu, W.: Multiple instance detection network with
  online instance classifier refinement. In: Proceedings of the IEEE Conference
  on Computer Vision and Pattern Recognition. pp. 2843--2851 (2017)

\bibitem{tang2018weakly}
Tang, P., Wang, X., Wang, A., Yan, Y., Liu, W., Huang, J., Yuille, A.: Weakly
  supervised region proposal network and object detection. In: Proceedings of
  the European conference on computer vision (ECCV). pp. 352--368 (2018)

\bibitem{tang2016large}
Tang, Y., Wang, J., Gao, B., Dellandr{\'e}a, E., Gaizauskas, R., Chen, L.:
  Large scale semi-supervised object detection using visual and semantic
  knowledge transfer. In: Proceedings of the IEEE Conference on Computer Vision
  and Pattern Recognition. pp. 2119--2128 (2016)

\bibitem{tao2018zero}
Tao, Q., Yang, H., Cai, J.: Zero-annotation object detection with web knowledge
  transfer. In: Proceedings of the European Conference on Computer Vision
  (ECCV). pp. 369--384 (2018)

\bibitem{tarvainen2017mean}
Tarvainen, A., Valpola, H.: Mean teachers are better role models:
  Weight-averaged consistency targets improve semi-supervised deep learning
  results. In: Advances in neural information processing systems. pp.
  1195--1204 (2017)
 
\bibitem{tan2020efficientdet}
Tan, Mingxing, Ruoming Pang, and Quoc V. Le. "Efficientdet: Scalable and efficient object detection." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2020.

\bibitem{vincent2008extracting}
Vincent, P., Larochelle, H., Bengio, Y., Manzagol, P.A.: Extracting and
  composing robust features with denoising autoencoders. In: Proceedings of the
  25th international conference on Machine learning. pp. 1096--1103 (2008)

\bibitem{wang2018towards}
Wang, K., Yan, X., Zhang, D., Zhang, L., Lin, L.: Towards human-machine
  cooperation: Self-supervised sample mining for object detection. In:
  Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition. pp. 1605--1613 (2018)

\bibitem{wang2015unsupervised}
Wang, X., Gupta, A.: Unsupervised learning of visual representations using
  videos. In: Proceedings of the IEEE International Conference on Computer
  Vision. pp. 2794--2802 (2015)

\bibitem{wu2019detectron2}
Wu, Y., Kirillov, A., Massa, F., Lo, W.Y., Girshick, R.: Detectron2.
  \url{https://github.com/facebookresearch/detectron2} (2019)

\bibitem{wu2018unsupervised}
Wu, Z., Xiong, Y., Yu, S., Lin, D.: Unsupervised feature learning via
  non-parametric instance-level discrimination. arXiv preprint arXiv:1805.01978
   (2018)

\bibitem{xie2019unsupervised}
Xie, Q., Dai, Z., Hovy, E., Luong, M.T., Le, Q.V.: Unsupervised data
  augmentation. arXiv preprint arXiv:1904.12848  (2019)

\bibitem{xie2019self}
Xie, Q., Hovy, E., Luong, M.T., Le, Q.V.: Self-training with noisy student
  improves imagenet classification. arXiv preprint arXiv:1911.04252  (2019)

\bibitem{yalniz2019billion}
Yalniz, I.Z., J{\'e}gou, H., Chen, K., Paluri, M., Mahajan, D.: Billion-scale
  semi-supervised learning for image classification. arXiv preprint
  arXiv:1905.00546  (2019)

\bibitem{yan2017weakly}
Yan, Z., Liang, J., Pan, W., Li, J., Zhang, C.: Weakly-and semi-supervised
  object detection with expectation-maximization algorithm. arXiv preprint
  arXiv:1702.08740  (2017)

\bibitem{yang2019detecting}
Yang, H., Wu, H., Chen, H.: Detecting 11k classes: Large scale object detection
  without fine-grained bounding boxes. In: Proceedings of the IEEE
  International Conference on Computer Vision. pp. 9805--9813 (2019)

\bibitem{yang2019towards}
Yang, K., Li, D., Dou, Y.: Towards precise end-to-end weakly supervised object
  detection network. In: Proceedings of the IEEE International Conference on
  Computer Vision. pp. 8372--8381 (2019)

\bibitem{yang2019activity}
Yang, Z., Mahajan, D., Ghadiyaram, D., Nevatia, R., Ramanathan, V.: Activity
  driven weakly supervised object detection. In: Proceedings of the IEEE
  Conference on Computer Vision and Pattern Recognition. pp. 2917--2926 (2019)

\bibitem{yarowsky1995unsupervised}
Yarowsky, D.: Unsupervised word sense disambiguation rivaling supervised
  methods. In: 33rd annual meeting of the association for computational
  linguistics. pp. 189--196 (1995)

\bibitem{zeng2019wsod2}
Zeng, Z., Liu, B., Fu, J., Chao, H., Zhang, L.: Wsod2: Learning bottom-up and
  top-down objectness distillation for weakly-supervised object detection. In:
  Proceedings of the IEEE International Conference on Computer Vision. pp.
  8292--8300 (2019)

\bibitem{zhou2019objects}
Zhou, X., Wang, D., Kr{\"a}henb{\"u}hl, P.: Objects as points. In: arXiv
  preprint arXiv:1904.07850 (2019)

\end{thebibliography}
